Enriching Wikidata with Linked Open Data

Large public knowledge graphs, like Wikidata, contain billions of statements about tens of millions of entities, thus inspiring various use cases to exploit such knowledge graphs. However, practice shows that much of the relevant information that fits users' needs is still missing in Wikidata, while current linked open data (LOD) tools are not suitable to enrich large graphs like Wikidata. In this paper, we investigate the potential of enriching Wikidata with structured data sources from the LOD cloud. We present a novel workflow that includes gap detection, source selection, schema alignment, and semantic validation. We evaluate our enrichment method with two complementary LOD sources: a noisy source with broad coverage, DBpedia, and a manually curated source with a narrow focus on the art domain, Getty. Our experiments show that our workflow can enrich Wikidata with millions of novel statements from external LOD sources with high quality. Property alignment and data quality are key challenges, whereas entity alignment and source selection are well-supported by existing Wikidata mechanisms. We make our code and data available to support future work.

==> sections/old_results.tex <==
\section{Results}
\label{sec:results}

\subsection{Overall enrichment results}




The results of our batch enrichment are shown in Table~\ref{tab1}. In total, the enrichment procedure yields 14.66 million validated statements for the 862 Wikidata properties. The statement enrichment rate is 16.56\%, which means that the enriched graph has 16.56\% more statements than the original graph. These novel statements cover a total of 8.33 million new entities. The coverage of entities for the 862 properties increased by 12.07\%, extending the original 60.72 million with 8.33 million more. 


Comparing the two external KGs, we observe that most of the added statements are contributed by DBpedia. DBpedia overall covers many more statements and entities than Getty, and its enrichment rate for the properties found is much higher than Getty (16.55\% vs 0.08\%). We note that out of 862 Wikidata properties with a value-type constraint, 516 properties can be aligned with DBpedia and 3 can be mapped with Getty. The remaining properties cannot be mapped with our method, which means that none of their known value pairs could be mapped to a pair in the external knowledge graphs. This is not surprising, as some of the Wikidata properties only have a small number of statements. In fact, 300 properties in Wikidata have under 200 statements, and 69\% of these properties have no mapped statements in DBpedia. 

% do not correspond to pairs in the external graphs, which might mean that the external graphs do not have that property, or that the alignment of the entities is suboptimal. \filip{let's pick some examples here to give at least anecdotal evidence about which of the two is more probable.} \bohui{There are 300 properties that each has less than 200 statements in Wikidata and 206 of them do not have mapped results in DBpedia.}


% 30 million novel statements about 16.23 million entities that previously had no value for a given property. 
% %new entities among . \move{I edit it and add numbers} 
% The value-type constraint validation of these newly found values results in 8.32 million semantically valid values for 16.23 million new entities, corresponding to a semantic compatibility rate of 51.28\%. The enrichment rate is 10.38\%, as the originally represented 71.8 million entities are now enriched with 8.32 million additional ones. 



% DBpedia overall covers many more statements and entities than Getty, and its enrichment rate for the properties found is much higher than Getty (10.38\% vs 0.08\%). Meanwhile, the correctness rate of the two sources is similar, with slight advantage of Getty (54.84\% vs 51.25\%).
% The remaining properties cannot be mapped with our method, because their known value pairs do not correspond to pairs in the external graphs, which might mean that the external graphs do not have that property, or that the alignment of the entities is suboptimal. 



% \begin{table}[!t]
% \centering
% \caption{Batch enrichment results when using DBpedia (DBP), Getty (GTY), and both graphs. $n_*$ represents total numbers of entities (Qnodes), $r_*$ stands for rates, and $s_*$ shows numbers of statements. In total, we consider 862 properties, 516 of which can be mapped to DBpedia, and 3 to Getty.} % \filip{is the average computed only based on the mapped properties? Yes. Actually the results are based on the mapped results, 516 in total.}}
% \label{tab1}
% \begin{center}
% \begin{tabular}{c | r r r r | r r | r r}
% % \begin{tabularx}{\textwidth}{>{\centering}p{0.13\textwidth}>{\centering}p{0.14\textwidth}>{\centering}p{0.12\textwidth}>{\centering}p{0.12\textwidth}>{\centering}p{0.12\textwidth}>{\centering}p{0.1\textwidth}>{\centering}p{0.1\textwidth}>{\centering\arraybackslash}p{0.1\textwidth}}
% \toprule
% & \multicolumn{2}{c}{Statements} & \multicolumn{4}{c}{Entities} \\
%  & $n_k$ & $n_{new}$ & $n_c$ & $n_v$ & $s_{new}$ & $s_c$ & $r_e$ & $r_c$\\
% \midrule
% \bf DBP & 71,869,914 & 16,234,798 & 8,320,744 & 8,621,064 & 30,123,341 & 14,648,000 & 16.66\% & 48.63\% \\
% \bf GTY & 7,452,668 & 10,514 & 5,766 & 4,752 & 10,518 & 5,766 & 0.14\% & 54.82\% \\ 
% \bf Both & 71,869,914 & 16,240,276 & 8,328,761 & 8,621,064 & 30,133,859 & 14,653,766 & 16.54\% & \bf 48.63\% \\
% \bottomrule
% \end{tabular}
% \end{center}
% \end{table}


% \begin{figure}
% \centering
% \includegraphics[width=0.66\textwidth]{images/ratio.png}
% \caption{Scatter plot distribution of ratios for enrichment $r_n$, correct $r_c$. Each dot corresponds to a single property. Properties are shown in a descending order according to their ratios and the x-axis has been } \label{fig4}
% \end{figure}


\begin{table}[!t]
\centering
\caption{Batch enrichment results when using DBpedia, Getty, and both KGs. $s_*$ shows numbers of statements, $n_*$ represents total numbers of entities (Qnodes), and $r_e$ stands for enrichment rates of statements or entities. In total, we consider 862 properties. $|p^\prime|$ shows the numbers of properties mapped to each of the KGs.} % \filip{is the average computed only based on the mapped properties? Yes. Actually the results are based on the mapped results, 516 in total.}}
\label{tab1}
\begin{center}
\begin{tabular}{c | r | r r r | r r r }
% \begin{tabularx}{\textwidth}{>{\centering}p{0.13\textwidth}>{\centering}p{0.14\textwidth}>{\centering}p{0.12\textwidth}>{\centering}p{0.12\textwidth}>{\centering}p{0.12\textwidth}>{\centering}p{0.1\textwidth}>{\centering}p{0.1\textwidth}>{\centering\arraybackslash}p{0.1\textwidth}}
\toprule
& & \multicolumn{3}{c}{\bf Statements} & \multicolumn{3}{c}{\bf Entities} \\
 & $|p^\prime|$ & $s_f$ & $s_c$ & $r_e$ & $n_k$ & $n_f$ & $n_c$\\
\midrule
\bf DBpedia & 516 & 30,123,723 & 14,657,999 & 16.55\% & 60,721,109 & 16,238,966 & 8,330,083 \\
\bf Getty & 3 & 10,518 & 5,766 &  0.08\% & 7,452,668 & 10,514 & 5,766  \\ 
\bf Both & 516 & 30,134,241 & 14,663,765 & 16.56\%  & 60,721,109 & 16,244,444 & 8,338,100  \\
\bottomrule
\end{tabular}
\end{center}
\end{table}


\begin{figure}[!t]
     \centering
     \begin{subfigure}[b]{0.49\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/r_e.png}
        %  \caption{}
        %  \label{fig3a}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.49\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/r_c.png}
        %  \caption{$y=3sinx$}
        %  \label{rates}
     \end{subfigure}
     \caption{Scatter plot distribution of rates for (a) enrichment $r_e$ and (b) semantic compatibility $r_c$ of statements, for DBpedia. Each dot corresponds to a single property. Properties are shown in a descending order according to their rates.}
     \label{rates}
\end{figure}


% Finally, the agreement rate is 4.60\% - indicating that only 1 in 20 values in Wikidata can be found in external graphs like DBpedia.\filip{discuss what to do with this rate}




% For the overall results, the first question we care about would be: what is the effect of the enrichment? 
% We select 862 properties from Wikidata with all of them have value-type constraints. 

The semantic compatibility rates in Table~\ref{tab1} demonstrate the value of the automatic validation done by our method. The enrichment method is able to retrieve 30 million statements in total, but only under half of them satisfy the constraints of the semantic validation. As all properties in this experiment have a value-type constraint, we infer that most of the discarded statements did not satisfy the expected semantic type.
% we can see this validation as a check of entity's semantic type. 
On a subject entity level, the enrichment procedure initially found new information for 16.24M subjects that previously lacked statements for a given property; yet, only 8.33M of these subjects had new objects that satisfy the value type constraint of the property. The compatibility ratios are similar for both Getty and DBpedia, which is surprising, considering that DBpedia has been largely extracted automatically and is error-prone, whereas Getty is well-curated and considered an authority. We provide explanation for this result in section~\ref{ssec:queries}.

% for statements an$s_c$

\subsection{Property-based analysis}

Figure \ref{rates} provides a scatter plot of the distribution of enrichment and compatibility ratios for all properties, for DBpedia. We observe that our enrichment method is able to contribute new values for nearly all properties, and it doubles the coverage of statements for nearly a third of the properties for which we have alignment. Meanwhile, the semantic compatibility of the newly found results is relatively high for most properties: more than half of the properties have at least 80\% valid new statements. We also note a steep decline in the $r_c$ curve, which means that a small portion of the properties have mostly semantically incompatible values. The semantic validation is thus an essential component of a knowledge enrichment architecture, as it enables fine-grained distinction between statements that satisfy and statements that violate a property constraint.
% certain constraint for a property.

% This motivates the need for using automated property-based methods for semantic validation.


\begin{table}[!t]
\centering
\caption{The 5 results with highest and lowest enrichment rate of DBpedia enrichment for the mapping properties. } %, count in Qnode.} %\filip{add property labels once you validate}}
\label{tab2}
\begin{center}
\begin{tabular}{c | r r | r r |r r r }
\toprule
Property & $s_f$ & $s_c$ & $r_e$ & $r_c$ & $n_k$ & $n_f$ & $n_c$ \\
\midrule
exclave of (\texttt{P500}) & 986,448 & 957,512 & 99.99\% & 97.07\% & 101 & 398,021 & 395,176 \\
running mate (\texttt{P6149}) & 15,777 & 8,822 & 99.98\% & 55.92\% & 2 & 9,957 & 6,201 \\
game artist (\texttt{P3080}) & 188,048 & 99,312 & 99.87\% & 52.81\% & 85 & 182,263 & 95,977 \\
supported sports team (\texttt{P6758}) & 306,768 & 288,752 & 99.86\% & 94.13\% & 341 & 46,899 & 44,136\\
ancestral home (\texttt{P66}) & 809,309 & 806,602 & 99.83\% & 99.67\% & 1,291 & 465,942 & 465,381 \\
% \texttt{P5389} permanent resident of & 1,244 & 465,866 & 441,553 & 95,757 & 99.72\% & 94.78\%\\ 
\midrule
family name (\texttt{P734}) & 15 & 9 & 0.00\% & 60.00\% & 2,863,889 & 15 & 9\\
research site (\texttt{P6153}) & 47 & 28 & 0.01\% & 59.57\% & 107,745 & 33 & 20  \\
located on astronomical body (\texttt{P376}) & 1 & 1 & 0.01\% & 100\% & 9,135 & 1 & 1\\
connecting service (\texttt{P1192}) & 26,928 & 3 & 0.02\% & 0.01\% & 12,181 & 16,810 & 3\\
twinned administrative body (\texttt{P190}) & 10 & 10 & 0.02\% & 100\% & 16,822 & 10 & 10 \\
\bottomrule
\end{tabular}
\end{center}
\end{table}

% The correct rate shows 63.33\% in average and 83.84\% in median of the found results in DBpedia Infobox passed semantic validation. And for the consistency of the results, there are in average ()\% of the results between Wikidata and Getty agrees. Given that the same information may represent in different format in these two graphs and DBpedia Infobox may contain much more information than value in Wikidata, we can primarily say the quality of the results reaches a relatively high level. 

The five properties with highest and lowest enrichment rate ($r_e$) are listed in Table \ref{tab2}. 
% \move{Results have been checked.} \filip{todo:comment once Bohui has validated the table}
We observe that the top 5 properties have an enrichment rate of over 99.8\%, and contribute 2,306,350
% \filip{how many} \bohui{2,306,350}
statements for around one million new entities. This represents a large influx of new values for these properties: for instance, the property \texttt{game artist}, which originally had values for 341 entities in Wikidata, is enriched with 289k new statements for 44k entities that had no value for that property. 
The semantic compatibility rate for these properties is generally high, ranging from 52 to 99\%. 
Meanwhile, the five properties with lowest enrichment rate, such as family name (\texttt{P734}), have enrichment rates of nearly 0\% and contribute only 51 validated statements in total. Upon manual inspection, we see that the low enrichment rate for these properties is due to several factors: (1) sparse population of the external graph - the Wikidata property family name (\texttt{P734}) is mapped to \texttt{property:familyName}, for which DBpedia has only 176 statements in total; (2) datatype inconsistency between DBpedia and Wikidata - e.g., 104 values for the property \texttt{property:familyName} in DBpedia are strings which does not match the expected datatype of a Qnode in Wikidata; (3) semantic incompatibility - for some properties, like connecting service (\texttt{P1192}) in Table~\ref{tab2}, DBpedia is able to provide many novel statements, but most of them have a semantic type (e.g., train operating company) that does not match the expected ones in Wikidata (train category or service for \texttt{P1192}).

% with Wikidata

% is mainly 

% \bohui{mainly due to the shortage of data within these properties in DBpedia. For instance, the Wikidata property \texttt{family name (P734)} is mapped to \texttt{property:familyName} in DBpedia which has 57 agreed statements with Wikidata. We can infer that the mapped property of DBpedia is correct. But even add up all the values with other datatypes like strings, this property only has 176 statements in DBpedia which is still a relatively small amount. The other reasons such as DBpedia has different preferred datatype for representing the values so they can not be mapped to Qnodes and perform value-type constraint validation. For example when the values represent people or information related to personal information, DBpedia will provide more strings rather than Qnodes. The low semantic consistency rate is also a problem like connecting service (\texttt{P1192}).}

% \bohui{the mapped property in DBpedia is \texttt{property:familyName} which has 57 agreed statements with Wikidata The incompatible values are due to }\filip{Bohui to check and give example - could be another property}.


%  Among these property pairs, we can further check the most and least 5 ones which could give us a more detailed information. Table. \ref{tab2} shows the top 5 properties with the most and the least $r_e$. We can find that for the top 5 results, (). While for the least top 5 results, ().


% We analyze batch query results on a total of 862 properties in Wikidata with DBpedia and 6 properties with Getty, by comparing the results between two graphs and evaluate the runtime. We also explore the quality of the new finding results through the results of validation.

% \subsubsection{DBpedia} 
% The statistics of DBpedia results are shown on 







% \begin{table}[!htb]
% \centering
% \caption{The lest 5 results (enrichment rate) of DBpedia enrichment for the mapping properties, count in Qnode.}
% \label{tab9}
% \begin{center}
% \begin{tabularx}{\textwidth}{>{\centering}p{0.13\textwidth}>{\centering}p{0.14\textwidth}>{\centering}p{0.12\textwidth}>{\centering}p{0.12\textwidth}>{\centering}p{0.1\textwidth}>{\centering}p{0.1\textwidth}>{\centering}p{0.12\textwidth}>{\centering\arraybackslash}p{0.12\textwidth}}
% \toprule
%  & Known & New & Correct & $r_e$ & $r_c$ & Incorrect & Agree\\
% \midrule
% P734 & 2,863,889 & 8,011 & 202 & 7,816 & 0.0071\% & 2.52\% & 89\\
% P641 & 1,735,485 & 5,922 & 128 & 5,797 & 0.0074\% & 2.16\% & 157\\
% P376 & 9,135 & 1 & 1 & 0 & 0.0109\% & 100\% & 276\\
% P6153 & 107,745 & 33 & 20 & 14 & 0.0186\% & 60.61\% & 1\\
% P59 & 1,023,970 & 227 & 222 & 6 & 0.0217\% & 97.80\% & 655\\
% \bottomrule
% \end{tabularx}
% \end{center}
% \end{table}


\subsection{Enrichment scenarios}
\label{ssec:queries}

To gain further insight, we consider 10 user query scenarios over Wikidata. We use DBpedia to enrich information about: movies (\texttt{Q11424}) with cost (\texttt{P2130}), founding year (\texttt{P571}) of universities (\texttt{Q3918}), spouses (\texttt{P26}) of politicians (\texttt{Q82955}), and 
industry (\texttt{P452}) of companies (\texttt{Q783794}). We enrich the following information about artists by querying Getty: date of birth (\texttt{P569}), date of death (\texttt{P570}), place of birth (\texttt{P19}), place of death (\texttt{P20}), nationality (\texttt{P27}), and gender (\texttt{P21}). 
% For the first 4 properties, we select DBpedia Infobox as enrichment source, and select Getty Vocabularies for the last 6 ones.


\begin{table}[!t]
\centering
\caption{Enrichment for ten example user queries. We enrich with DBpedia for the following four queries: movies (\texttt{11424}) with cost (\texttt{P2130}), founding year (\texttt{P571}) of universities (\texttt{Q3918}), spouses (\texttt{P26}) of politicians (\texttt{Q82955}), and industry (\texttt{P452}) of company (\texttt{Q783794}). We enrich with Getty for six queries about artists: date of birth (\texttt{P569}), date of death (\texttt{P570}), place of birth (\texttt{P19}), place of death (\texttt{P20}), country of citizenship (\texttt{P27}), and sex or gender (\texttt{P21}). To validate the data, we use value-type constraints when possible. In the remaining cases, we perform datatype validation. The queries for which we have value type constraint are marked with an asterisk.}
\label{tab3}
\begin{center}
\begin{tabular}{l | r r | r r | r r r r | r}
\toprule
& \multicolumn{4}{c}{Statements} & \multicolumn{5}{c}{Subjects} \\
Query & $s_f$ & $s_c$ & $r_e$ & $r_c$ & $n_k$ & $n_u$ & $n_f$ & $n_c$ & $r_r$ \\
\midrule
M-Cost & 19,701 & 1,517 & 31.25\% & 7.70\% & 3,330 & 300,208 & 18,336 & 1,517 & 0.50\% \\
U-FY & 53 & 25 & 0.18\% & 47.17\% & 13,385 & 2,317 & 50 & 25 & 1.08\% \\
P-Spo  & 58,733 & 1,250 & 3.28\% & 2.12\% & 30,281 & 593,029 & 39,438 & 1,238 & 0.21\% \\
C-Ind* & 4,257 & 512 & 2.58\% & 12.03\% & 16,088 & 265,773 & 3,493 & 435 & 0.16\% \\
\hline
A-DoB & 8,243 & 8,243 & 8.30\% & 100\% & 83,993 & 8,217 & 8,217 & 8,217 & 100\% \\
A-DoD & 19,674 & 6,001 & 7.23\% & 30.50\% & 70,837 & 21,373 & 19,654 & 5,995 & 28.05\% \\
A-PoB* & 2,939 & 2,939 & 4.29\% & 100\% & 64,680 & 27,530 & 2,939 & 2,939 & 10.68\% \\
A-PoD* & 2,554 & 2,554 & 4.82\% & 100\% & 49,757 & 42,453 & 2,556 & 2,556 & 6.02\% \\
A-CoC* & 5,026 & 271 & 0.34\% & 5.40\% & 69,291 & 22,919 & 5,019 & 271 & 1.18\% \\
A-SoG & 532 & 532 & 0.59\% & 100\% & 89,188 & 3,022 & 495 & 495 & 16.38\% \\
\midrule
% Average & 49,083.00 & 128,684.10 & 10,019.70 & 7,833.70 & 2,787.20 & 16.95\% & 78.18\% & 12,171.20 & 8,389.70\\
Total & 121,712 & 23,844 & 4.33\% & 19.59\% & 490,830 & 1,286,841 & 100,197 & 23,688 & 1.84\% \\
\bottomrule
\end{tabular}
\end{center}
\end{table}



The results are shown in Table~\ref{tab3}. We see that Wikidata contains property values for tens of thousands of queried entities, but also that many entities lack expected values. For instance, most movie costs and company industries are missing in Wikidata. By using DBpedia, we are able to retrieve 0.5\% of the missing property values for movie costs, enriches the original data by 31.25\%.
The enrichment and retrieval rates for the remaining DBpedia queries are generally low.
% Meanwhile, the enrichment procedure is only able to retrieve 25 new values for 25 new entities when it comes to founding years of universities, confirming our earlier observation that the enrichment procedure with the two selected graphs has a variable effect, largely dependent on the query needs.
As for the remaining six queries, we observe that Getty is able to retrieve much higher portions of the missing values, as apparent from the retrieval rate $r_r$.
We note that for some properties, such as \texttt{sex or gender} and \texttt{founding year}, Wikidata already has fairly complete knowledge (e.g., 96.72\% Qnodes already have value for property gender), which leaves little room for enrichment. For this artist property, Getty is able to retrieve 495 (16.38\%) of the missing values for which Wikidata did not have a value.
By doing so, Getty enriches Wikidata by around 20 thousand new values.

Semantic compatibility rates are largely responsible for the different trends between DBpedia and Getty. Owing to its automatic creation method, the enrichment with DBpedia has low compatibility rates.
% \filip{in table 3, the results seem strange. i remember we had many values that did not pass semantic validation of datatype in dbpedia. How come we have nearly 100\% r\_c for m-cost, u-fy, and p-spo?}. 
% , largely due to the low semantic compatibility rates of its results. 
In most cases, DBpedia provides results scattered across multiple datatypes, which is incompatible with Wikidata's semantics.
For instance, most of the candidate values for company industries (2,389 out of 3,493) are strings, which violates Wikidata's datatype validation. 
% Upon inspection, we see that this is because there are 2,389 industry values in DBpedia represented as strings which we will not count in value-type constraint validation thus not shown in the table. 
% These strings have agreed statements with Wikidata thus the novel statements there can be potentially correct. For example \texttt{COM DEV International (Q1024012)} has inferred novel results from DBpedia as \texttt{'Telecommunications'@en} and this is correct according to Wikidata but not recorded here.
% Our enrichment procedure is able to bring 121,712 new statements for these queries, 84 thousand of which pass the semantic validation. These new statements provide property values for 78 thousand subjects that lacked values for that property before, out of the 1.3 million entities in total for which Wikidata lacked value according to their type. Overall, the retrieval rate is \filip{how much}
% The enrichment is most effective for obtaining costs of movies and spouses of politicians through Wikidata, whose enrichment rates are 84 and 57\%, respectively. Meanwhile, the enrichment procedure is only able to retrieve 53 new values for 43 new entities when it comes to founding years of universities, confirming our earlier observation that the enrichment procedure with the two selected graphs has a variable effect, largely dependent on the query needs. The six artist queries for which we use Getty yield nearly 50 thousand new statements, around 20 thousand of which are valid.
% These results again show that for certain queries it is essential to use semantic validation in order to ensure that the expected semantics is compatible between the source and the external knowledge graph. While certain queries, such as spouses of politicians or place of birth of artists, have nearly perfect compatibility score, others have much lower rates. In the case of DBpedia, we observe a notably low compatibility score when enriching company industries. Upon inspection, we see that this is because \bohui{there are 2389 industry values in DBpedia represented as strings which we will not count in value-type constraint validation thus not shown in the table. These strings have agreed statements with Wikidata thus the novel statements there can be potentially correct. For example \texttt{COM DEV International (Q1024012)} has inferred novel results from DBpedia as \texttt{'Telecommunications'@en} and this is correct according to Wikidata but not recorded here}. 
In the case of Getty, we expect perfect semantic rates, which holds for 4 out of 6 properties. The lower compatibility rate for date of death (30.5\%) is because most of the newly found dates are surprisingly future dates (2022 and beyond). The country of citizenship property yields new values for five thousand new entities, but only 5\% of those fit the value type constraints in Wikidata. This is because the aligned property in Getty is \texttt{gvp:nationality}, which has similar semantics but has a non-identical expected value type. Upon inspection, we find that 81.27\% of the nationality values in Getty are instances of the class \texttt{culture of an area (Q19958368)}, rather than the expected value of a country in Wikidata. For example, a German artist in Getty would have a nationality \texttt{culture of Germany (Q1979615)} rather than the country \texttt{Germany (Q183)}.



\begin{table}[!t]
\centering
\caption{Results of property mapping with our schema alignment procedure. We use `+' to separate hops in multi-hop paths.}
\label{tab6}
\begin{center}
\begin{tabular}{c|c}
\toprule
\Centering\bfseries WD & \Centering\bfseries External graph \\
\midrule 
M-Cost & \texttt{property:budget} \\
U-FY & \texttt{property:established}\\
P-Spo & \texttt{property:spouse} \\
C-Ind & \texttt{property:industry}\\ \hline
A-DoB & \texttt{foaf:focus+gvp:biographyPreferred+\textbf{gvp:estStart}+gvp:structured\_value} \\
A-DoD & \texttt{foaf:focus+gvp:biographyPreferred+gvp:estEnd+gvp:structured\_value} \\
A-PoB & \texttt{foaf:focus+gvp:biographyPreferred+schema:birthPlace+skos:exactMatch} \\
A-PoD & \texttt{foaf:focus+gvp:biographyPreferred+schema:deathPlace+skos:exactMatch} \\
A-CoC & \texttt{foaf:focus+gvp:nationalityPreferred+skos:exactMatch} \\
A-SoG & \texttt{foaf:focus+gvp:biographyPreferred+schema:gender+skos:exactMatch} \\
\bottomrule
\end{tabular}
\end{center}
\end{table}

Finally, we see that the alignment procedure yields a reasonable path in the external graph for each of the ten queries (Figure~\ref{tab6}).
% , we show the top-1 most frequent associated property path in the external graphs. For all ten queries, . 
Direct connections in Wikidata (e.g., spouse - P26) often correspond to direct connections in DBpedia (\texttt{property:spouse}). Each Wikidata property corresponds to a 3- or 4-hop path in Getty, owing to the more complex formalism in Getty to separate different roles of a given entity, and different biographies that could correspond to a role. Yet, we note that this might lead to additional noise during the enrichment procedure. For example, when enriching dates of death, we find three paths which yield relatively high set of values. Replacing \texttt{gvp:biographyPreferred} in the optimal path with \texttt{gvp:biographyNonPreferred} yields 12,558 newly covered entities, and replacing it with \texttt{gvp:EventPreferred} results in 2,707 newly covered entities. The top-1 path chosen by our method yields the highest increase of covered entities (19,654) and the highest number of correctly validated entities (13,659 as opposed to 9,647 and 68 for the two concurrent paths). 





% \begin{table}[!t]
% \centering
% \caption{Path 1: \texttt{[foaf:focus, gvp:biographyPreferred, gvp:estEnd, gvp:structured\_value]}; Path 2: \texttt{[foaf:focus, gvp:biographyNonPreferred, gvp:estEnd, gvp:structured\_value]}; Path 3: \texttt{[foaf:focus, gvp:eventPreferred, gvp:estEnd, gvp:structured\_value]}}
% \label{tab4}
% \begin{center}
% \begin{tabularx}{\textwidth}{>{\centering}p{0.18\textwidth}>{\centering}p{0.1\textwidth}>{\centering}p{0.08\textwidth}>{\centering}p{0.11\textwidth}>{\centering}p{0.11\textwidth}>{\centering}p{0.08\textwidth}>{\centering}p{0.09\textwidth}>{\centering}p{0.09\textwidth}>{\centering\arraybackslash}p{0.09\textwidth}}
% \toprule
% Property & Known & Novel & Validated & Violated & $r_e$ & $r_c$ & $r_a$ & Value per node\\
% \midrule 
% Path 1 & 70,837 & \textbf{19,654} & \textbf{5,995} & \textbf{13,659} & \textbf{7.80\%} & 30.50\% & \textbf{78.47\%} & 1.001\\
% Path 2 & 70,837 & 12,588 & 2,941 & 9,647 & 3.99\% & 23.36\% & 67.04\% & 1.558\\
% Path 3 & 70,837 & 2,707 & 2,639 & 68 & 3.59\% & \textbf{97.49\%} & 1.89\% & 0.998\\
% \bottomrule
% \end{tabularx}
% \end{center}
% \end{table}


% The reason is that Getty uses different way to represent nationality with Wikidata. In the found new nationality results in Getty, 81.27\% of the nationality represented as instance of "culture of an area" (\texttt{Q19958368}). For example, a German artist in Wikidata would have nationality "Germany" (\texttt{Q183}), while in Getty his/her nationality would be "culture of Germany" (\texttt{Q1979615}). The gender property has the most number of known records in Wikidata (96.72\% Qnodes already have value for property gender), thus Getty could not provide that much enrichment on this property.



% \filip{comment on the following: (1) how many are missing; (2) how many are found; (3) variance across the queries; (4) variance across the graphs;}
% This is essential because in some cases the external graphs contain incorrectly extracted information. For instance, only 1,238 out of the \filip{how many} spouse values in DBpedia are Qnodes, and only 3,589 out of \filip{how many} values for budget of films are structured literals.\filip{budget vs cost}

% Par 2: here are the paths that we used

% Par 3: semantic validation

% Par 4: 


% For situations with given property and known query entity range in Wikidata, we analyze 4 properties from Wikidata and their mapped property in DBpedia Infobox, see Table~\ref{tab1}. The properties including movies (\texttt{11424}) with cost (\texttt{P2130}),
% founding year (\texttt{P571}) of universities (\texttt{Q3918}), 
% spouses (\texttt{P26}) of politicians (\texttt{Q82955}), and 
% industry (\texttt{P452}) of company (\texttt{Q783794}). 
% For the first three user queries, the value of the property does not have value-type constraints. By checking the returned value manually, we can further apply validation through data type. For example, the value for \texttt{P2130} could be numbers and structured literals (numbers with currency), the value for \texttt{P26} can be Qnodes and strings (name of people). 
% The property \texttt{P452} has value-type constraints on Qnode results thus we can apply semantic validation. The results shows there are 435 Qnodes have the new results which passed semantic validation, and the correct rate reaches 29.73\%. 
% \move{The reason that our query still return strings, numbers and structured literals is that DBpedia Infobox will record dates information with spouses themselves, like the date or duration of the marriage. This time and date information is recorded in the graph as numbers, strings and structured literals. While check the data type can not meet our requirements, since the desired data type of each property largely depend on human insights, it can not generalize to batch query. Thus in our work, the validation would be mainly apply on Qnodes results.}

% The results of this 4 property give us a good insight of the quality of DBpedia Infobox, and this procedure could be easily generalized to other properties, even by creating a batch query consisted of multiple properties.

% \begin{table}[!t]
% \centering
% \caption{The statistics of 4 properties, count in Qnode. The Known column represent}
% \label{tab7}
% \begin{center}
% \begin{tabularx}{\textwidth}{>{\centering}p{0.12\textwidth}>{\centering}p{0.1\textwidth}>{\centering}p{0.32\textwidth}>{\centering}p{0.1\textwidth}>{\centering}p{0.1\textwidth}>{\centering}p{0.1\textwidth}>{\centering\arraybackslash}p{0.08\textwidth}}
% \toprule
% Wikidata Property & Entity Class & DBpedia Property & Known & Unknown & New & Agree\\
% \midrule
% P2130 & Q11424 & \texttt{property:budget} & 3,330 & 300,208 & 18,336 & 16\\
% P571 & Q3918 & \texttt{property:established} & 13,385 & 2,317 & 50 & 0\\
% P26 & Q82955 & \texttt{property:spouse} & 30,281 & 593,029 & 39,438 & 5,165\\
% P452 & Q783794 & \texttt{property:industry} & 16,056 & 265,805 & 3,493 & 4,281\\
% \bottomrule
% \end{tabularx}
% \end{center}
% \end{table}

% \begin{table}[!t]
% \centering
% \caption{Results of Getty enrichment for the properties, count in Qnode. There are 92,210 Qnodes in total that both in Wikidata and Getty Vocabularies. The Known column is counted through query for Wikidata. The New column represents the count of the new results we found from Getty. The Correct column represents the values among New that passed value-type constraint of Wikidata, and Incorrect columns counts those are not. Note that the validation of date of birth \& death is using custom validation by checking if the year is within the correct time range (e.g. before 2022) since date value do not have value-type constraint.}
% \label{tab3}
% \begin{center}
% \begin{tabularx}{\textwidth}{>{\centering}p{0.18\textwidth}>{\centering}p{0.1\textwidth}>{\centering}p{0.08\textwidth}>{\centering}p{0.11\textwidth}>{\centering}p{0.11\textwidth}>{\centering}p{0.08\textwidth}>{\centering}p{0.09\textwidth}>{\centering}p{0.09\textwidth}>{\centering\arraybackslash}p{0.09\textwidth}}
% \toprule
% Property & Known & Novel & Validated & Violated & $r_e$ & $r_c$ & $r_a$ & Value per node\\
% \midrule 
% A-Date of Birth & 83,993 & 8,217 & \textbf{8,217} & 0 & 8.91\% & \textbf{100\%} & \textbf{83.78\%} & 1.001\\
% Date of Death & 70,837 & \textbf{19,654} & 5,995 & \textbf{13659} & 7.80\% & 30.50\% & 78.47\% & 1.001\\
% Place of Birth & 64,680 & 2,939 & 2,939 & 0 & 4.35\% & \textbf{100\%} & 21.04\% & 1.000\\
% Place of Death & 49,757 & 2,556 & 2,556 & 0 & \textbf{4.89\%} & \textbf{100\%} & 25.32\% & 1.000\\
% Nationality & 69,291 & 5,019 & 271 & 4,752 & 0.39\% & 5.40\% & 0.47\% & 1.003\\
% Gender & \textbf{89,188} & 495 & 495 & 0 & 0.55\% & \textbf{100\%} & 9.88\% & 1.107\\
% \midrule
% Average & 71,291 & 4,489 & 2,090 & 2,400 & 3.00\% & 71.46\% & 32.24\% & 1.177\\
% Total & 427,746 & 26,933 & 12,538 & 14,399 & 2.85\% & 46.55\% & 33.05\% & / \\
% \bottomrule
% \end{tabularx}
% \end{center}
% \end{table}




% \begin{table}[!t]
% \centering
% \caption{Data type distribution on results of 4 sample properties. Data types with reasonable answers are \textbf{bold}.}\label{tab1}
% \begin{center}
% \begin{tabularx}{\textwidth}{>{\centering}p{0.15\textwidth}>{\centering}p{0.3\textwidth}>{\centering}p{0.12\textwidth}>{\centering}p{0.12\textwidth}>{\centering}p{0.16\textwidth}>{\centering\arraybackslash}p{0.08\textwidth}}
% \toprule
% Wikidata Property & DBpedia Property & Numbers & Strings & Structured literals & Qnodes\\
% \midrule
% P2130 & \texttt{property:budget} & \textbf{1,517} & \textbf{14,109} & \textbf{3,589} & 11\\
% P571 & \texttt{property:established} & \textbf{18} & 7 & \textbf{27} & 0\\
% P26 & \texttt{property:spouse} & 4,586 & \textbf{1,460} & 38,018 & \textbf{1,238}\\
% P452 & \texttt{property:industry} & 2 & \textbf{2,105} & 1 & \textbf{1,463}\\
% \bottomrule
% \end{tabularx}
% \end{center}
% \end{table}

% \subsubsection{Getty} Results from Getty reveal different results from DBpedia due to the ontology and overall (size) of data. As discussed in the method section, Getty Vocabularies have always been constructed to allow linking and ULAN, TGN, AAT are all linked to Wikidata. We select all people that have linked Wikidata Qnode and ULAN ID as the range of the entities, \move{with total size of 92,353 counting in ULAN IDs and 92,210 counting in Qnodes}. There exists the situation that one Qnode linked to multiple ULAN IDs, or multiple Qnodes linked to one ULAN IDs. The reason is that Getty may have two to three records for one person, and they may linked to one record in Wikidata. This also happens in Wikidata which could lead to multiple Qnodes linked to one ULAN ID. To align with Wikidata results, we will count the results in Qnodes. We select 6 properties from Getty which their value can be mostly linked to Wikidata directly through Qnodes. The statistics is shown in Table. \ref{tab1} and the property mapping between two graphs is shown in Table. \ref{tab6}. By comparing the property chains in Table. \ref{tab6}, we can see the chains have common parts at the beginning and the end of them. And there is a key property in the middle representing the meaning of the path. \move{For dates, Getty only provide strings of years so that we convert dates to year strings when performing property mapping.}

% We observe that since Wikidata already have complete information for artists, Getty can still provide \move{427,746 new results in total} and \move{71.46\%} of them can pass the validation. For date properties like date of birth and date of death, even if Wikidata already provide much information and leaves less space for enrichment, Getty still provide \move{a good amount of} new information. Especially for data of birth, Getty provides all the unknown results in Wikidata for the set of Qnodes, thus after enrichment there is no more unknowns in our queried Qnodes. The correct rate of date of death drops a lot because date of death in Getty contains dates later than this year (2021). For place of birth \& death, the new results from Getty which are TGN nodes all passed the validation. The compensation rate of these two properties are relatively high compared to the rest four properties, which shows the good quality and enrichment effect of TGN. For nationality of artists, the correct rate and number of agreed Qnode records drops to a quite low level compared to other properties. The reason is that Getty uses different way to represent nationality with Wikidata. In the found new nationality results in Getty, 81.27\% of the nationality represented as instance of "culture of an area" (\texttt{Q19958368}). For example, a German artist in Wikidata would have nationality "Germany" (\texttt{Q183}), while in Getty his/her nationality would be "culture of Germany" (\texttt{Q1979615}). The gender property has the most number of known records in Wikidata (96.72\% Qnodes already have value for property gender), thus Getty could not provide that much enrichment on this property. 

% \move{Results of Getty enrichment for the properties, count in Qnode. There are 92,210 Qnodes in total that both in Wikidata and Getty Vocabularies. The Known column is counted through query for Wikidata. The New column represents the count of the new results we found from Getty. The Correct column represents the values among New that passed value-type constraint of Wikidata, and Incorrect columns counts those are not. Note that the validation of date of birth \& death is using custom validation by checking if the year is within the correct time range (e.g. before 2022) since date value do not have value-type constraint.}

% \move{In most of our property mapping results, the frequency of the mapped property (chain) in the selected graph would be dominant thus the mapped property is obvious. But to evaluate the quality of property mapping, we provide an example in \ref{tab4} for date of death where 1) all of them can provide a certain amount of new results and 2) the size of the validated results are relatively close.}





\subsection{Time performance analysis}
We analyze the runtime of our batch query procedure over DBpedia. The results for the most critical steps of schema alignment, knowledge retrieval, and semantic validation are shown in Table~\ref{tab3}. 
We remind that these numbers exclude the initial step of transforming the DBpedia subject and object entities to Wikidata Qnodes, while the runtime of the remaining steps is negligible. 
% We focus on the procedure after user query for Wikidata, from schema alignment (entity resolution and property mapping), knowledge retrieval, semantic validation (datatype filtering, quality checking). 
Overall, our enrichment procedure is efficient:
enriching a single property takes around 4 minutes on average, including schema alignment and semantic validation.
Over half of the running time is spent on retrieving knowledge from DBpedia, while the critical phases of schema alignment and validation run quickly: schema alignment has a median runtime of 12 seconds, while semantic validation takes less than a minute on average. 
% retrieval of DBpedia Infobox. Property mapping will take () triples in total and make () times comparison. Similarly for quality checking which take () result triples and check each result in a list of () value-type constraints in average. While these two process take much less time compared to knowledge retrieval, which shows our procedure can get the results within reasonable time and run in a good efficiency.

\begin{table}[!t]
\centering
\caption{Runtime (in seconds) statistics of each step in the method of enriching Wikidata with DBpedia. We provide average, median, and standard deviation for each step over the 516 properties. As the entity resolution of entities was done beforehand, it is not factored into the statistics.}
\label{tab3}
\begin{center}
\begin{tabular}{c | r r |  r | r r | r}
\toprule
& \multicolumn{2}{c}{Schema Alignment} & {} & \multicolumn{2}{c}{Validation}& \\ 
{} & Entity & Property & Knowledge Retrieval & Datatype & Value-type & Total\\
\midrule
Average & 32.94 & 5.95 & 166.05 & 19.18 & 37.11 & 261.23\\
Median & 6.18 & 5.97 & 164.99 & 17.56 & 37.66 & 233.50\\
Std & 185.88 & 0.29 & 6.44 & 5.03 & 8.40 & 188.20\\
\bottomrule
\end{tabular}
\end{center}
\end{table}
